A sharp H\"{o}rmander condition for bilinear Fourier multipliers with Lipschitz singularities

This paper studies the $L^{p}$ boundedness of bilinear Fourier multipliers in the local $L^{2}$ range. We assume a H\"{o}rmander condition relative to a singular set that is a finite union of Lipschitz curves. The H\"{o}rmander condition is sharp with respect to the Sobolev exponent. Our setup generalizes the non-degenerate bilinear Hilbert transform but avoids issues of uniform bounds near degeneracy.

==> Tdef.tex <==


\begin{definition}[Continuous Whitney Decompositon]
    We define the bump function:
    \begin{equation}
        \rchi_\vbeta:=\Tr_\vbeta \Dil^\infty_{d_\Gamma\br{\vbeta}}\rchi.
    \end{equation}
    The \textbf{Whitney pieces} derived from the bump function with a suitable weight:
    \begin{equation}
        \widetilde{\rchi}_\vbeta:=X_{\Gamma}^{-1} \cdot \rchi_\vbeta
        \text{, where }
        X_{\Gamma}:= 
        \int_{V\setminus\Gamma} 
            \rchi_\vbeta
        \frac{d\mathcal{H}^n\br{\vbeta}}{d_\Gamma\br{\vbeta}^n}.
    \end{equation}
    Formally, we have:
    \begin{equation}
        \1_{V\setminus\Gamma}:= 
        \int_{V\setminus\Gamma} 
            \rchi_\vbeta
        \frac{d\mathcal{H}^n\br{\vbeta}}{d_\Gamma\br{\vbeta}^n}.
    \end{equation}
\end{definition}


\begin{definition}[Lipschitz curves]
    We choose the following specific form of orthonormal basis on $V$:
\begin{equation}
    \BR{
        \vu:=\frac{\operatorname{P}_{V}\ve_3}{|\operatorname{P}_{V}\ve_3|}=\frac{-\ve_1-\ve_2+2\ve_3}{\sqrt{6}},
        \vv:=\frac{\vu\times\vone}{|\vu\times\vone|}=\frac{-\ve_1+\ve_2}{\sqrt{2}}
    }\subset V.
\end{equation}


Fix a parameter \(\theta_\lip\in\Br{0,\frac{\pi}{6}-2\theta_{0}}\), where $\theta_{0}$ is a universal small constant.
We say $\Gamma \subset V$ is a Lipschitz curve  in \(\vu\) direction within \(\theta_\lip\) angle if for all $\vgamma\in\Gamma$
\begin{equation}
  \Gamma \cap \br{\vgamma+ \cC_{\lip}}=\varnothing,
    \hspace{1.5ex}\text{where}\hspace{1.5ex}
    \cC_{\lip}
    :=
    \left\{
        \vxi\in V
    \middle\vert
        \abs{\ang{\vu,\vxi}}<|\vxi|\cos\theta_\lip
    \right\}.
\end{equation}
\end{definition}

\begin{remark}
The above definition of Lipschitz curve coincide with the usual notion of Lipschitz condition when we view $\Gamma$ as the image of a function \(\gamma\) parametrized by the scaler projection of the function-value onto $\vu$. direction(\textcolor{red}{make the english better}.), then it's a Lipschitz curve with Lipschitz constant $\operatorname{tan}\theta_\lip$.
We may check that under the angle condition, \(\Gamma\) avoid the forbidden direction. In other words,
\begin{equation} 
  \{\operatorname{P}_{V}(\ve_{i}^{\perp}) \}_{i=1,2,3}
    \subseteq
    \cC_\lip
\end{equation}

For example, in the classcial BHT, $\{\vxi\in \mathbb{R}^{3} \vert \xi_{1}-\xi_{2}=0\}\cap V=\operatorname{P}_{V}\ve_3$.
\end{remark}


For convenience, we will work on following right-ward half-plane:
\begin{equation}
% \left\{
%     \begin{aligned}
        \H
        := 
        % &
        \left\{
            \vxi\in V
        \middle\vert
            \ang{\vv,\vxi}>0
        \right\}
        = 
        \left\{
            \vxi\in V
        \middle\vert
           \xi_1<\xi_2
        \right\}.
\end{equation}













==> Tsymbols.tex <==
\begin{itemize}
    \item $\bm{v}:$ Bold font for vectors. ex: $\bm{v}=(v_{1},v_{2},v_{3})$.
    \item $V:=\vone^{\perp}=(1,1,1)^{\perp}$: The hyperplane we work on.
    \item $\Gamma$: Singularity.
    \item $\operatorname{Tr}$: Translation operator. ex: $(\operatorname{Tr}_{a}f)(x):=f(x-a)$.
    \item $\operatorname{Mod}$: Modulation operator. ex: $(\operatorname{Mod}_{a}f)(x):=e^{2\pi iax}f(x)$.
    \item $\operatorname{Dil}$: Dilation Operator. ex: $(\operatorname{Dil}_{a}^{p}f)(x):a^{-\frac{n}{p}}f(\frac{x}{a})$.
    \item $\operatorname{P}$: Projection operator. ex: $\operatorname{P}_{V}(x)$ is the projection of $x$ on $V$.
    \item $\mathds{1}$: Characteristic function. ex: $\mathds{1}_{A}$, the characteristic function of $A$.
    \item $\rchi$: A Bump function.
    \item $\rchi_{\beta}$: A bump function adapted to $\beta$.
    \item $\widetilde{\rchi}_{\beta}$: A normalized bump function adapted to $\beta$.
    \item $\phi$: A Bump function larger than $\rchi$.
    \item $\phi_{\beta}$: $L^{\infty}$ normalized bump with frequency adapted to $\beta$. 
    \item $\varphi_{\beta}$:  $L^{2}$ normalized bump with frequency adapted to $\beta$. 
    \item  $\mathcal{C}_{Lip}$: Cones used to define Lipschitz curves.
    \item  $\mathcal{C}^{j}$: $j$-th standard cones.
    \item $\omega^{j}$: $j$-th standard truncated cones.
    \item $W_{\vgamma,t}^{j}$: $j$-th truncated cone with top $\vgamma$ and scale $t$.
\end{itemize}


==> dyadicTentest.tex <==
We demonstrate the main ideas of the proof of the main theorem with some estimate for a dyadic toy model in the Walsh phase plane that captures the essential organization in the phase plane.
We use notation as in \cite{} \todoct{insert some quartile operator paper}
for the Walsh phase plane.
In what follows, Walsh wave packets $\phi$ are $L^1$ normalized,
so that the brackets $\left<f,\phi\right>$ are averages of $f$.
Define 
\[\Lambda=\sum_{q=(I_1,I_2,I_3,\omega)\in Q}
a_q|I_q|
|\left< f_1,\phi_{I_1,\omega_1}\right>
\left< f_2,\phi_{I_2,\omega_2}\right>
\left< f_3,\phi_{I_3,\omega_3}\right>|,
\]
where $Q$ is the set of all quadruples 
\[q=(I_{q,1}, I_{q,2}, I_{q,3}, \omega_q)\] 
of dyadic intervals such that
\[|I_{q,3}|=|I_{q,2}|=|I_{q,3}|=:|I_q|\]
and 
\[|I_q||\omega_q|=4,\]
and $I_{q,i}$ are all contained in some dyadic interval $J_q$
of size $|J_q|=2^n|I_{q}|$ and both halves of $J_q$ contain
at least one of the $I_{q,i}$.
The interval $\omega_i$ is the $i$-th grandchild of $\omega$,
enumerating the four grandchildren from bottom to top.
The non-negative coefficients $a_q$ satisfy for each $i$ and each $I$,
$\omega$:
\[\sum_{q: I_{q,i}=I, \omega_q=\omega}|a_q|^2\le 1 .\]
All $f_i$ are characteristic functions of 
measurable sets of measure $1$. We claim that 
\begin{equation}\label{lambdaclaim}\Lambda \le Cn2^n.
\end{equation}


Define for each fixed $i$ trees in the sense of ordering of 
the quartiles $(I_i,\omega)$.
We do the standard tree decomposition for each $i$.
Assume for each $i$ we have a  collection $Q_i$ of quartiles
containing no tree of size larger than $2^k$.
For each $i$ we find a collection ${\bf T}_i$ of trees
such that removing these trees from $Q_i$ there are no trees
left in $Q_i$ of size larger than $2^{k-1}$ and
$$\sum_{T\in {\bf T}_i} |I_T| \le C 2^{-2k}.$$

Fix a tree $T\in \{T_i\}$ with top interval $I_T$. Let $S_T$ be the set of quadruples
$(I_1,I_2,I_3,\omega)$ such that the quartile $(I_i, \omega)$ is in $T$. We aim to show
\begin{equation}\label{treeclaim}
\Lambda_{S_T} \le C 2^{3k} n2^n|I_T|,
\end{equation}
where $\Lambda_{S_T}$ is defined by restricting the sum in 
$\Lambda$ to $S_T$. This will prove \eqref{lambdaclaim}
by summing over all $i$, all trees in $T_i$, and all $k\le 0$.


We will estimate separately the sum over quadruples in $S_T$
with $|I_q|>2^{-n}|I_T|$ and with $|I_q|\le 2^{-n}|I_T|$.

First consider $|I_q|>2^{-n}|I_T|$.
We estimate, using that $T_i$ is a subset of $P_k$,
\[\sum_{q\in S_T, |I_q|>2^{-n}|I_T|}
a_q|I_q|
|\left< f_1,\phi_{I_1,\omega_1}\right>
\left< f_2,\phi_{I_2,\omega_2}\right>
\left< f_3,\phi_{I_3,\omega_3}\right>|
\]
\[\le \sum_{q\in S_T, |I_q|>2^{-n}|I_T|}
|a_q||I_q|2^{3k}
\]
\[\le \sum_{I_1\subset I_T,  |I_1|>2^{-n}|I_T|}
2^n|I_1|2^{3k}.
\]
In the last line we used that there are at most $2^{2n}$ triples $I_1,I_2,I_3$
for given $I_1$, because $I_2$ and $I_3$ are contained in $J_q$,
and we used Cauchy Schwartz and the bound on $a_q$.
Next, we use that the $|I_1|$ with $I_1\subset I_T$ at fixed scale add up
to $|I_T|$ and that there are $n$ possible scales in the sum to obtain 
for the last display
\[\le 
n2^n|I_T|2^{3k}.
\]
This proves the analog of \eqref{treeclaim} for the sum over quadruples
with large $I_q$.



Now consider $|I_q|\le 2^{-n}|I_T|$.
We split the tree into its different types and without
loss of generality consider the $1$-overlapping tree $T_1$.






We estimate
\[\sum_{q=(I_1,I_2,I_3,\omega_1)\in S_{T_1}: |I_q|\le 2^{-n}|I_T|}
a_q|I_q|
|\left< f_1,\phi_{I_1,\omega_1}\right>
\left< f_2,\phi_{I_2,\omega_2}\right>
\left< f_3,\phi_{I_3,\omega_3}\right>|
\]
\[\le 2^k 
\sum_{(I_1,I_2,I_3,\omega_1)\in S_{T_1},|I_q|\le 2^{-n}|I_T|}
a_q|I_q|
|\left< f_2,\phi_{I_2,\omega_2}\right>
\left< f_3,\phi_{I_3,\omega_3}\right>|
\]
\[\le 2^k 
\sum_{I_1}
(\sum_{I_2\subset J_q}|I_2||\left< f_2,\phi_{I_2,\omega_2}\right>||^2)^{1/2}
(\sum_{I_3\subset J_q}|I_3||\left< f_3,\phi_{I_3,\omega_3}\right>||^2)^{1/2}.
\]
Here we have used that $J_q$ and $\omega$  are  determined by $I_1$
for quadruples in the tree $T$, we have used that $I_2,I_3\subset J_s$,
and we have used the bound on $a_q$ by doing a Cauchy-Schwartz.
Using that $J_q$ contains $2^n$ intervals of length $I_1$ and
regrouping the sum by intervals $J$, we estimate the last display by
\[\le 2^k 2^n
\sum_{J}
(\sum_{I_2\in J}|I_2||\left< f_2,\phi_{I_2,\omega_2}\right>|^2)^{1/2}
(\sum_{I_3\in J}|I_3||\left< f_3,\phi_{I_3,\omega_3}\right>|^2)^{1/2}.
\]
By the smallness assumption on $I_q$, we have that $J$ is at most as large as $I_T$ and thus contained in $I_T$. Doing Cauchy Schwartz over the sum of $J$, we estimate the last display by

\[\le 2^k 2^n
(\sum_{I_2\in I_T}|I_2||\left< f_2,\phi_{I_2,\omega_2}\right>|^2)^{1/2}
(\sum_{I_3\in I_T}|I_3||\left< f_3,\phi_{I_3,\omega_3}\right>|^2)^{1/2}
\]
\[\le 2^{3k} 2^n |I_T| .\]
This proves the analog of \eqref{treeclaim} for the sum over quadruples
with small $I_q$.


==> geometry_of_cones.tex <==
\begin{proposition}\label{prop_buffer_zone}
    There's a positive constant \(\epsilon_0 =\frac{1}{\sqrt{6}}\wedge\br{\frac{\sqrt{6}}{3}\sin\theta_0}\) such that
    \begin{equation}
        \left\{
            \vxi\in\H
        \middle\vert
            \frac{\abs{\xi_i}}{\abs{\vxi}}<\epsilon_0
        \right\}
        \subset
        \cC^i
        ,\hspace{1.5ex}\forall i.
    \end{equation}
\end{proposition}

\begin{proof}[proof of Lemma \ref{subconelemma}]
    Consider the affine transformation: \(\vxi \mapsto \frac{\vxi-\vgamma_W}{\abs{W}}\). Since \(\Gamma\mapsto \frac{\Gamma-\vgamma_W}{\abs{W}}\) is again a \(\vu\)-oriented Lipschitz curve angled within \(\frac{\pi}{6}-2\theta_0\), it suffices to consider the case where \(W=\omega\). Moreover, by symmetry, it's enough to prove:
    \begin{equation}
        \Omega^+_{\leq 0}\cap \pi_{\epsilon,i}\br{\omega^j}\subset \rho \omega\hspace{1.5ex}\text{whenever}\hspace{1.5ex}i\circlearrowright j.
    \end{equation}
    Let \(\vxi\in\Omega^+_{\leq 0}\cap \pi_{\epsilon,i}\br{\omega^j}\). By assumption, we can find \(\vbeta\in\omega^j\) such that
    \begin{equation}
        \frac{\abs{\beta_i-\xi_i}}{\abs{\vbeta}+\abs{\vxi}}
        \leq
        \frac{\abs{\beta_i-\xi_i}}{d_\Gamma\br{\vbeta}+d_\Gamma\br{\vxi}}
        <\epsilon \ll\epsilon_0.
    \end{equation}
    \begin{itemize}
        \item We first show that \(\vxi\in\cC\).
            Assume the alternative: \(\vxi\notin\cC\). Clearly, \(\vbeta,\vxi\notin\cC^i\). By \textit{proposition \ref{prop_buffer_zone}}, we have:
            \begin{equation}
                \frac{\abs{\beta_i}}{\abs{\vbeta}},\frac{\abs{\xi_i}}{\abs{\vxi}}\geq \epsilon_0.
            \end{equation}
            Yet, due to the orientation \(i\circlearrowright j\),
            \begin{equation}
                \abs{\beta_i-\xi_i}=\abs{\beta_i}+\abs{\xi_i}
                \geq 
                \epsilon_0 \br{\abs{\vbeta}\vee\abs{\vxi}}
                \eqsim 
                \epsilon_0 \br{\abs{\vbeta}+\abs{\vxi}}.
            \end{equation}
            Choosing small enough \(\epsilon\) gives the following contradiction:
            \begin{equation}
                \epsilon_0\lesssim \frac{\abs{\beta_i-\xi_i}}{\abs{\vbeta}+\abs{\vxi}}<\epsilon \ll\epsilon_0.
            \end{equation}
        \item Next, we show that \(\ang{\vv,\vxi}>\rho\) for small enough \(\rho\ll\epsilon_0\). We again proceed by assuming the opposition: \(\ang{\vv,\vxi}\leq \rho\). Since \(\vxi\in\cC\), we have:
        \begin{equation}
            \abs{\vxi}\eqsim\ang{\vv,\vxi} \leq \rho\ll\epsilon_0.
        \end{equation}
        On the other hand, \(\vbeta\in\omega^j\) implies that
        \begin{equation}
            \abs{\vbeta}\eqsim\ang{\vv,\vbeta}>1\gg \epsilon_0.
        \end{equation}
        Therefore, we have:
        \begin{equation}
            \frac{\abs{\beta_i-\xi_i}}{\abs{\vbeta}}\eqsim \frac{\abs{\beta_i-\xi_i}}{\abs{\vbeta}+\abs{\vxi}}<\epsilon \ll \epsilon_0.
        \end{equation}
        Yet, again \(\vbeta\notin\cC^i\), we have \(\frac{\abs{\beta_i}}{\abs{\vbeta}}\geq \epsilon_0\) and thus,
        \begin{equation}
            \frac{\abs{\xi_i}}{\abs{\vbeta}}
            \geq
            \frac{\abs{\beta_i}}{\abs{\vbeta}}-\frac{\abs{\beta_i-\xi_i}}{\abs{\vbeta}}
            \eqsim
            \frac{\abs{\beta_i}}{\abs{\vbeta}}\geq \epsilon_0.
        \end{equation}
        This, for small enough \(\rho\), leads to the following contradiction:
        \begin{equation}
            \epsilon_0< \epsilon_0\abs{\vbeta}
            \lesssim
            \abs{\xi_i}\leq\abs{\vxi}
            \lesssim
            \rho \ll\epsilon_0.
        \end{equation}
    \end{itemize}
    Combining both bullet points, we conclude that \(\vxi\in\rho\omega\).
\end{proof}


Due to symmetry, we shall focus on the \(i\circlearrowright j\) scenario. For the same settings, we have the following 

\begin{proof}[proof of Lemma \ref{scalebddlemma}]
     Using again the affine transform argument, we may assume 
    \begin{equation}
        \vgamma=\vzero \hspace{1.5ex}\text{and}\hspace{1.5ex}\ang{\vv,\vbeta}=1.
    \end{equation}
    As a direct consequence, we have:
    \begin{equation}
        d_\Gamma\br{\vbeta} \leq \abs{\vbeta}\eqsim \ang{\vv,\vbeta}=1.
    \end{equation}
    On the other hand, since
    \begin{equation}
        \vbeta'\in\Omega^+_{\leq 0}\cap \pi_{\epsilon,i}\br{\vbeta}
        \subset \Omega^+_{\leq 0}\cap \pi_{\epsilon,i}\br{\omega^j}\subset \rho \omega,
    \end{equation}
    we must have:
    \begin{equation}
        1\underset{\theta_0}{\eqsim}\rho \leq \ang{\vv,\vbeta'}\underset{\theta_0}{\eqsim}d_\Gamma\br{\vbeta'}.
    \end{equation}
     Combine what we obtain, we get:
    \begin{equation}
        d_\Gamma\br{\vbeta}\underset{\theta_0}{\lesssim}d_\Gamma\br{\vbeta'}.
    \end{equation}
    This completes the first part. If in addition, \(\vbeta'\in\vgamma'+\cC^j\) with \(\gamma_3\leq 0\), we also have:
    \begin{equation}
        \abs{\vbeta'-\vgamma'}\underset{\theta_0}{\eqsim}d_\Gamma\br{\vbeta'}
        % \underset{\theta_0}{\eqsim}\ang{\vv,\vbeta'}\eqsim\abs{\vbeta'}
        .
    \end{equation}
    Yet, since \(\vbeta'\notin \vgamma'+\cC^i\),
    \begin{equation}
        \frac{\abs{\beta'_i-\gamma'_i}}{d_\Gamma\br{\vbeta'}}\underset{\theta_0}{\eqsim}\frac{\abs{\beta'_i-\gamma'_i}}{\abs{\vbeta'-\vgamma'}}\in\left(\epsilon_0,1\right].
    \end{equation}
    Now, we combine the first part of the corollary and the fact that \(\vbeta'\in \pi_{\epsilon,i}\br{\vbeta}\) to obtain:
    \begin{equation}
        \frac{\abs{\beta'_i-\beta_i}}{d_\Gamma\br{\vbeta'}}\underset{\theta_0}{\eqsim}
        \frac{\abs{\beta'_i-\beta_i}}{d_\Gamma\br{\vbeta'}+d_\Gamma\br{\vbeta}}
        <\epsilon\ll\epsilon_0.
    \end{equation}
    Lastly, the triangle inequality yields the result:
    \begin{equation}
        \frac{\abs{\beta_i-\gamma'_i}}{d_\Gamma\br{\vbeta'}}\lesseqgtr
        \frac{\abs{\beta_i'-\gamma_i'}}{d_\Gamma\br{\vbeta'}}\pm\frac{\abs{\beta'_i-\beta_i}}{d_\Gamma\br{\vbeta'}}
        \underset{\theta_0}{\eqsim}
        \frac{\abs{\beta_i'-\gamma_i'}}{d_\Gamma\br{\vbeta'}}
        \underset{\theta_0}{\eqsim}1.
    \end{equation}
    This completes the second part of the lemma.
\end{proof}

==> geometry_of_tents.tex <==
\begin{proof}[Proof of Lemma \ref{strdis}]
    
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem_sym_tent_cover}] 
    
\end{proof}

==> proof_of_maincor.tex <==
\textcolor{red}{Need to adapt to the current version.}
    \begin{equation}\label{cor}
        \|m_{\beta ,t}\|_{H^{s}}= \left\| \int_{\mathbb{R}^{2}}\widetilde{m}(t(\xi_{1}-\xi_{2}))\widehat{\psi}(\xi_{1}-\xi_{2})\widehat{\varphi}(\xi_{1}+\xi_{2}-\frac{\beta}{t})e^{2\pi i(\xi_{1}x_{1}+\xi_{2}x_{2})}d\xi_{1}d\xi_{2} \cdot (1+|(x_{1},x_{2})|^{2})^{\frac{s}{2}}\right\|_{L^{2}_{x}}
    \end{equation}
    In the inner integral, we have
    \begin{equation}
        \int_{\mathbb{R}^{2}}\left(\widetilde{m}(t(\xi_{1}-\xi_{2}))\widehat{\psi}(\xi_{1}-\xi_{2})e^{2\pi i(\xi_{1}-\xi_{2})(\frac{x_{1}-x_{2}}{2})} \right)\cdot \left(\widehat{\varphi}(\xi_{1}+\xi_{2}-\frac{\beta}{t})e^{2\pi i(\xi_{1}+\xi_{2})(\frac{x_{1}+x_{2}}{2})} \right)d\xi_{1}d\xi_{2}
    \end{equation}
Take supreme in \eqref{cor}, the we have
\begin{equation}
\begin{aligned}
 &\underset{\beta \in \mathbb{R},t>0}{\operatorname{sup}}\left\| (1+|(x_{1},x_{2})|^{2})^{\frac{s}{2}}k_{t}(\frac{x_{1}-x_{2}}{2}) (M_{\frac{\beta}{t}}\varphi)(\frac{x_{1}+x_{2}}{2})\right\|_{L^{2}_{x}}\\
    \lesssim &\underset{\beta \in \mathbb{R},t>0}{\operatorname{sup}} \left\|(1+|\frac{x_{1}-x_{2}}{2}|^{2})^{\frac{s}{2}}k_{t}(\frac{x_{1}-x_{2}}{2}) \cdot (1+|\frac{x_{1}+x_{2}}{2}|^{2})^{\frac{s}{2}}(M_{\frac{\beta}{t}}\varphi)(\frac{x_{1}+x_{2}}{2})\right\|_{L^{2}_{x}}\\
    \lesssim &\underset{\beta \in \mathbb{R},t>0}{\operatorname{sup}} \|\widehat{k_{t}}\|_{H^{s}}\cdot \|T_{\frac{\beta}{t}}\widehat{\varphi}\|_{H^{s}}\lesssim \underset{\beta \in \mathbb{R},t>0}{\operatorname{sup}} \|\widehat{k_{t}}\|_{H^{s}} < +\infty
 \end{aligned}
\end{equation}
where $k_{t}=\mathcal{F}^{-1}({D^{\infty}_{t^{-1}}m\widehat{\psi}})$.
